Sparse Reconstruction via The Reed-Muller Sieve

This paper introduces the Reed Muller Sieve, a deterministic measurement matrix for compressed sensing. The columns of this matrix are obtained by exponentiating codewords in the quaternary second order Reed Muller code of length $N$. For $k=O(N)$, the Reed Muller Sieve improves upon prior methods for identifying the support of a $k$-sparse vector by removing the requirement that the signal entries be independent. The Sieve also enables local detection; an algorithm is presented with complexity $N^2 \log N$ that detects the presence or absence of a signal at any given position in the data domain without explicitly reconstructing the entire signal. Reconstruction is shown to be resilient to noise in both the measurement and data domains; the $\ell_2 / \ell_2$ error bounds derived in this paper are tighter than the $\ell_2 / \ell_1$ bounds arising from random ensembles and the $\ell_1 /\ell_1$ bounds arising from expander-based ensembles.

==> conc.tex <==
In compressed sensing the entries of the measurement vector constitute evidence for the presence or absence of a signal at any given location in the data domain. We have shown that the Reed Muller sieve is able to identify the support set without requiring that the signal entries be independent. We have also demonstrated feasibility of local decoding where attributes of the signal are deduced from the measurements without explicitly reconstructing the full signal. Our reconstruction algorithms are resilient to noise and the $\ell_2/ \ell_2$ error bounds are tighter than the $\ell_2 / \ell_1$ bounds arising from random ensembles and the $\ell_1 /\ell_1$ bounds arising from expander-based ensembles.

==> old_proof.tex <==
Let $Q$ be a binary symmetric matrix and let $E$ be the null space of $Q$. Let $X$ be an $\ell$ dimensional subspace of $\mathbb{F}_2^m$ and let $f \in \mathbb{F}_2^m$. If $$S=\sum_{x \in X+f}\imath^{xQx^\top+2bx^\top}\,\mbox{where }b\in \mathbb{F}_2^m,$$
then either $S=0$ or $$S^2=\imath^{fQf^\top+2bf^\top} \imath^{z_1Qz_1^\top+2(b+fQ)z_1^\top}2^{\ell+\mbox{dim}(X\cap E)},$$
where $z_1\in X$ is a solution to $z_1Q=d_Q$ and $d_Q$ is the main diagonal of $Q$.
\end{proposition}
\begin{proof}
The general case reduces quickly to the case $f=0$ where
$$S^2=\sum_{x,y} \imath^{(x+y)Q(x+y)^\top+2xQy^\top+2b(x+y)^\top}.$$
Changing variables to $z=x+ y$ and $y$ gives
$$S^2=\sum_z \imath^{zQz^\top+2bz^\top}\sum_y (-1)^{(d_Q+zQ)y^\top}.$$
Since the diagonal of $Q$ is contained in the row space of $Q$ there exits a solution $z_1$ to $zQ=d_Q$. If there is no solution $z_1$ in $X$ then $S=0$. Otherwise 
$$S^2=2^{\ell} \imath^{z_1Qz_1^\top+2z_1b^\top} \sum_{e\in E\cap X} \imath^{eQe^\top+2be^\top}.$$
The map $e\rightarrow eQe^\top+2be^\top$ is a linear map from $E$ to $2\,\mathbb{Z}_4$. If this map is the zero map then $S^2\nobreak=\nobreak2^{\ell+\mbox{dim}(E\cap X)} \imath^{z_1Qz_1^\top+2z_1b^\top}$, and if not then $S=0$. 
\end{proof}


==> sieve_old <==
\begin{thebibliography}{10}

\bibitem{CRT1}
E.~Cand\`{e}s, J.~Romberg, and T.~Tao,
\newblock ``Stable signal recovery from incomplete and inaccurate
  measurements,''
\newblock {\em Comm. Pur. Appl. Math., vol. 59, no. 8 , pp. 1207-1223.}, 2006.

\bibitem{Donoho}
D.~Donoho,
\newblock ``Compressed {S}ensing,''
\newblock {\em IEEE Trans. Inform. Theory, vol. 52, no. 4, pp. 1289-1306},
  2006.

\bibitem{CT}
E.~Cand\`{e}s and T.~Tao,
\newblock ``Near optimal signal recovery from random projections: Universal
  encoding strategies,''
\newblock {\em IEEE Trans. Inform. Theory, vol. 52, no. 12, pp. 5406-5425},
  Dec. 2006.

\bibitem{CRT2}
E.~Cand\`{e}s, J.~Romberg, and T.~Tao,
\newblock ``Robust uncertainty principles: {E}xact signal reconstruction from
  highly incomplete frequency information,''
\newblock {\em IEEE Trans. Inform. Theory, vol. 52, no. 2, pp. 489-509}, 2006.

\bibitem{greed}
J.~Tropp,
\newblock ``Greed is {G}ood: {A}lgorithmic {R}esults for {S}parse
  {A}pproximation,''
\newblock {\em IEEE Trans. Inform. Theory, vol. 50, no. 10, pp. 2231-2242},
  Oct. 2004.

\bibitem{NT}
D.~Needell and J.~A. Tropp,
\newblock ``Co{S}a{M}{P}: Iterative signal recovery from incomplete and
  inaccurate samples.,''
\newblock {\em Appl. Comp. Harm. Anal. vol. 26, no. 3, pp. 301-321}, May 2009.

\bibitem{CP07}
E.~Cand\`es and J.~Plan,
\newblock ``Near-ideal model selection by $\ell_1$ minimization,''
\newblock {\em Ann. Stat. , vol. 37, pp. 2145-2177}, 2009.

\bibitem{dantzig}
E.~Cand\`{e}s and T.~Tao,
\newblock ``The {D}antzig selector: Statistical estimation when $p$ is much
  larger than $n$,''
\newblock {\em Ann. Stat.}, vol. 35, pp. 2392--2404, 2007.

\bibitem{DM}
W.~Dai and O.~Milenkovic,
\newblock ``Subspace pursuit for compressive sensing: {C}losing the gap between
  performance and complexity,''
\newblock {\em to appear in IEEE Trans. Inform. Theory}, 2009.

\bibitem{IR}
P.~Indyk and M.~Ruzic,
\newblock ``Near-optimal sparse recovery in the $\ell1$ norm,''
\newblock {\em 49th Annual IEEE Symposium on Foundations of Computer Science,
  pp. 199-207}, 2008.

\bibitem{sina}
S.~Jafarpour, W.~Xu, B.~Hassibi, and R.~Calderbank,
\newblock ``{Efficient compressed Sensing using Optimized Expander Graphs},''
\newblock {\em IEEE Trans. Inform. Theory, vol. 55, no. 9, pp. 4299-4308},
  2009.

\bibitem{best}
A.~Cohen, W.~Dahmen, and R.~DeVore,
\newblock ``Compressed sensing and best $k$-term approximation,''
\newblock {\em Am. Math. Soc. vol. 22, pp. 211-231}, 2009.

\bibitem{strip}
R.~Calderbank, S.~Howard, and S.~Jafarpour,
\newblock ``Construction of a large class of matrices satisfying a statistical
  isometry propery,''
\newblock {\em To appear in the Comp. Sensing Special Issue of IEEE Jr. Sel.
  Topics Sig. Proc}, 2009.

\bibitem{tech1}
R.~Calderbank, S.~Howard, and S.~Jafarpour,
\newblock ``{C}hirp {R}econstruction {A}lgorithm for {S}parse {R}econstruction
  with $\ell_2 /\ell_2$ {R}ecovery {G}uarantees,''
\newblock {\em \bl{Princeton Univ. Tech. Report. Manuscript available at
  \textit{http://www.cs.princeton.edu/$\sim$sina/rm$\_$sieve.pdf}}}, 2010.

\bibitem{DG}
P.~Delsarte and J.~M. Goethals,
\newblock ``Alternating bilinear forms over {GF}$(q)$,''
\newblock {\em Jr. Comb. Theory, vol. 19, pp. 26-50}, 1975.

\bibitem{H}
A.~R.~Hammons Jr., P.~V. Kumar, A.~R. Calderbank, N.~J.~A. Sloane, and P.~Sole,
\newblock ``The $\mathbb{Z}_4$-linearity of {K}erdock {C}odes, {P}reparata,
  {G}oethals, and related codes,''
\newblock {\em IEEE Trans. on Inform. Theory. vol. 40, no. 2, pp. 301-319},
  March 1994.

\bibitem{omid}
D.~Omidiran and M.~Wainwright,
\newblock ``High-dimensional subset recovery in noise: Sparsified measurements
  without loss of statistical efficiency,''
\newblock {\em IEEE International Symposium on Information Theory (ISIT)},
  2008.

\bibitem{HSC}
S.~Howard, R.~Calderbank, and S.~Searle,
\newblock ``A fast reconstruction algorithm for deterministic compressive
  sensing using second order {R}eed-{M}uller codes,''
\newblock {\em Conference on Information Sciences and Systems (CISS), pp. 11 -
  15}, March 2008.

\end{thebibliography}

